Dataset Meta-Learning from Kernel Ridge-Regression

One of the most fundamental aspects of any machine learning algorithm is the training data used by the algorithm. We introduce the novel concept of $\epsilon$-approximation of datasets, obtaining datasets which are much smaller than or are significant corruptions of the original training data while maintaining similar model performance. We introduce a meta-learning algorithm called Kernel Inducing Points (KIP) for obtaining such remarkable datasets, inspired by the recent developments in the correspondence between infinitely-wide neural networks and kernel ridge-regression (KRR). For KRR tasks, we demonstrate that KIP can compress datasets by one or two orders of magnitude, significantly improving previous dataset distillation and subset selection methods while obtaining state of the art results for MNIST and CIFAR-10 classification. Furthermore, our KIP-learned datasets are transferable to the training of finite-width neural networks even beyond the lazy-training regime, which leads to state of the art results for neural network dataset distillation with potential applications to privacy-preservation.

==> experiments_log.tex <==
Table A1: (MNIST, KIP and LS vs baselines)
FC1, ntk parameterization
https://xm2a.corp.google.com/experiments/17623795
https://xm2a.corp.google.com/experiments/17628789

RBF
https://xm2a.corp.google.com/experiments/17579822


Table A2: (CIFAR, KIP and LS vs baselines)
RBF:
17570785 (old, did not have seeds, channel shift = 10)
18133970


FC1:
17629931 (except for 5k and 10k images, channel shift=20)
17629931 (5k, 10k, no augs)
17503429 (5k, 10k with augs, SOTA)


Table A3: (random sample of images on CIFAR10)
17658293
18104897
-------
18104897
18109001 (linear)


----------------

Table A4:


For general kernels, we make the following simple observation concerning the optimal output of \algname.

17569725 (rbf on all of cifar10 due to Jaehoon)

Fig A1 (kernel to kernel transfer):
17507848

-------------

Table A5:


10 Images:
https://xm2a.corp.google.com/experiments/17587392
wid: 44, 74

100 images:
https://xm2a.corp.google.com/experiments/17412618
wid: 86, 116

200 images:
https://xm2a.corp.google.com/experiments/17412618
wid: 128, 158

Tables A7-A10:
XM_ID_CIFAR10_kip = 18156829 # KIP
XM_ID_MNIST_kip1 = 18156782 # KIP
XM_ID_MNIST_kip2 = 18157272 # KIP
XM_ID_CIFAR10_natural_baseline_mse = 18194081  # mse only
XM_ID_MNIST_natural_baseline_mse = 18194000  # mse only
XM_ID_CIFAR10_natural_baseline_xent = 18207593
XM_ID_MNIST_natural_baseline_xent = 18207603
